On the eta-invariant of certain nonlocal boundary value problems

Motivated by the work of Vishik on the analytic torsion we introduce a new class of generalized Atiyah-Patodi-Singer boundary value problems. We are able to derive a full heat expansion for this class of operators generalizing earlier work of Grubb and Seeley. As an application we give another proof of the gluing formula for the eta invariant. Our class of boundary conditions contains as special cases the usual (nonlocal) Atiyah-Patodi-Singer boundary value problems as well as the (local) relative and absolute boundary conditions for the Gauss-Bonnet operator.

==> rrdummy.tex <==
%
% CMR font family for math symbols by Ingo Eichenseher
%
\font\tenrr=cmbx10  scaled \magstep1
\font\sevenrr=cmbx7 scaled \magstep1
\font\fiverr=cmbx5 scaled \magstep1

\newfam\rrfam
\textfont\rrfam=\tenrr
\scriptfont\rrfam=\sevenrr
\scriptscriptfont\rrfam=\fiverr

\def\A{{\fam\rrfam A}}
\def\B{{\fam\rrfam B}}
\def\C{{\fam\rrfam C}}
\def\D{{\fam\rrfam D}}
\def\E{{\fam\rrfam E}}
\def\F{{\fam\rrfam F}}
\def\G{{\fam\rrfam G}}
\def\H{{\fam\rrfam H}}
\def\I{{\fam\rrfam I}}
\def\J{{\fam\rrfam J}}
\def\K{{\fam\rrfam K}}
\def\L{{\fam\rrfam L}}
\def\M{{\fam\rrfam M}}
\def\N{{\fam\rrfam N}}
\def\O{{\fam\rrfam O}}
\def\P{{\fam\rrfam P}}
\def\Q{{\fam\rrfam Q}}
\def\R{{\fam\rrfam R}}
%\def\S{{\fam\rrfam S}}
\def\T{{\fam\rrfam T}}
\def\U{{\fam\rrfam U}}
\def\V{{\fam\rrfam V}}
\def\W{{\fam\rrfam W}}
\def\X{{\fam\rrfam X}}
\def\Y{{\fam\rrfam Y}}
\def\Z{{\fam\rrfam Z}}
\def\one{{\fam\rrfam 1}}

